Wavelet Latent Diffusion (Wala): Billion-Parameter 3D Generative Model with Compact Wavelet Encodings

Large-scale 3D generative models require substantial computational resources yet often fall short in capturing fine details and complex geometries at high resolutions. We attribute this limitation to the inefficiency of current representations, which lack the compactness required to model the generative models effectively. To address this, we introduce a novel approach called Wavelet Latent Diffusion, or WaLa, that encodes 3D shapes into wavelet-based, compact latent encodings. Specifically, we compress a $256^3$ signed distance field into a $12^3 \times 4$ latent grid, achieving an impressive 2427x compression ratio with minimal loss of detail. This high level of compression allows our method to efficiently train large-scale generative networks without increasing the inference time. Our models, both conditional and unconditional, contain approximately one billion parameters and successfully generate high-quality 3D shapes at $256^3$ resolution. Moreover, WaLa offers rapid inference, producing shapes within two to four seconds depending on the condition, despite the model's scale. We demonstrate state-of-the-art performance across multiple datasets, with significant improvements in generation quality, diversity, and computational efficiency. We open-source our code and, to the best of our knowledge, release the largest pretrained 3D generative models across different modalities.

==> Sections/AB_Dataset.tex <==
\section{Dataset details}
\begin{table}[h]
\centering
\begin{tabular}{|c|c|}
Dataset & Number of meshes \\
\hline
3dfuture & 16,560 \\
abc & 988,681 \\
abo & 7,953 \\
buildingnet & 1,849 \\
coma & 20,465 \\
deformingthings4d & 121,123 \\
fg3d & 25,546 \\
fusion & 162,653 \\
github & 4,946,342 \\
gso & 1,030 \\
house3d & 500 \\
infinigen & 96,318 \\
modelnet40 & 12,311 \\
objaverse & 798,118 \\
shapenet\_v2 & 51,209 \\
smal & 23,000 \\
smpl & 58,758 \\
thingi10k & 9,951 \\
thingiverse & 3,231,391 \\
toy4k & 3,994 \\
\hline
Total & 10,577,752 \\
\end{tabular}
\caption{The 10 million 3D shape dataset.}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|}
Dataset & Number of meshes \\
\hline
3dfuture & 16,560 \\
abc & 512,060 \\
abo & 6,804 \\
buildingnet & 1,849 \\
coma & 20,465 \\
deformingthings4d & 121,123 \\
fg3d & 25,552 \\
fusion & 46,528 \\
github & 1,492,718 \\
house3d & 499 \\
infinigen & 112,587 \\
modelnet40 & 12,311 \\
objaverse & 763,327 \\
shapenet\_v2 & 51,209 \\
smal & 23,000 \\
smpl & 58,759 \\
thingi10k & 4,790 \\
thingiverse & 1,184,241 \\
toy4k & 3,998 \\
\hline
Total & 4,458,380 \\
\end{tabular}
\caption{A training subset of the 10 million 3D shape dataset excluding meshes with small file sizes.}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|}
Dataset & Number of meshes \\
\hline
3dfuture & 10,000 \\
abc & 10,000 \\
abo & 6,644 \\
buildingnet & 1,812 \\
coma & 10,000 \\
deformingthings4d & 10,000 \\
fg3d & 10,000 \\
fusion & 10,000 \\
github & 10,000 \\
house3d & 490 \\
infinigen & 10,000 \\
modelnet40 & 10,000 \\
objaverse & 10,000 \\
shapenet\_v2 & 10,000 \\
smal & 10,000 \\
smpl & 10,000 \\
thingi10k & 4,682 \\
thingiverse & 10,000 \\
toy4k & 3,912 \\
\hline
Total & 157,540 \\
\end{tabular}
\caption{A training slice of the 4.4 million 3D shape dataset including up to 10,000 shapes per dataset.}
\end{table}

==> tables/inference_timestep.tex <==
% \begin{table}
% \tiny
% \centering
% {\caption{We quantitatively evaluate the performances of generation models with different inference time steps.}%
% \label{tab:timestep_comp}
% \begin{tabular}{c|c|ccccccccccc}
% \toprule
%  &  & \multicolumn{11}{c}{Inference Time Step (t)} \\
% \multirow{-2}{*}{Model}       & \multirow{-2}{*}{Metrics} & t=10 & t=12 & t=100 & t=3 & t=15 & t=20 & t=30 & t=40 & t=50 & t=70 & t=5         \\
% \midrule
% \multirow{2}{*}{Point Cloud}  & LFD $\downarrow$  & 1454.62 & 1476.37 & 1500.64 & 2965.79 & 1429.26 & 1389.64 & 1409.61 & 1408.93 & 1413.77 & 1417.12 & 1574.28            \\
%                               & IoU $\uparrow$    & 0.8552  & 0.8564  & 0.8525  &             \\
% \midrule
% \multirow{2}{*}{Single-view}  & LFD $\downarrow$ & 2892.78 & 2885.85 & 2942.61 & 3166.60 & 2906.67 & 2894.96 & 2891.91 & 2911.02 & 2900.16 & 2923.45 & 2908.45 \\
%                               & IoU $\uparrow$   & 0.5961  & 0.5934  & 0.5733  &                \\
% \midrule
% \multirow{2}{*}{Multi-view}   & LFD $\downarrow$ & 1585.10 & 1564.41 & 1556.83 & 2371.45 & & 1507.04 & 1538.63 & 1525.69 & 1529.07 & 1527.60 &               \\
%                               & IoU $\uparrow$   & 0.81098 & 0.8083  & 0.7960 &                \\
% \midrule
% \multirow{2}{*}{Voxels ()}    & LFD $\downarrow$ & 1970.10 & 1949.43 & 2035.14 & 2449.85 & 1935.44 & 1906.15 & 1931.36 & 1939.85 & 1932.56 & 1950.61 & 1872.56                \\
%                               & IoU $\uparrow$   & 0.7454  & 0.7457  & 0.7307  &                \\
% \midrule
% \multirow{2}{*}{4 depth}      & LFD $\downarrow$ & & & & 2430.07 & & 1414.29 & 1408.15 & 1421.16 & 1420.80 & 1428.63  \\
%                               & IoU $\uparrow$   & & & &               \\
% \midrule
% \multirow{2}{*}{6 depth}      & LFD $\downarrow$ & & & & 2588.48 & & 1348.32 & 1350.47 & 1353.88 & 1355.54& 1360.20 \\
%                               & IoU $\uparrow$   \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

% \begin{table}
% \tiny
% \centering
% {\caption{We quantitatively evaluate the performances of generation models with different inference time 
% steps.}%
% \label{tab:timestep_comp}
% \begin{tabular}{c|c|ccccccccccc}
% \toprule
%  &  & \multicolumn{11}{c}{Inference Time Step (t)} \\
% \multirow{-2}{*}{Model}       & \multirow{-2}{*}{Metrics} & t=10 & t=12 & t=100 & t=3 & t=15 & t=20 & t=30 & t=40 & t=50 & t=70 & t=5         \\
% \midrule
% \multirow{2}{*}{Point Cloud}  & LFD $\downarrow$  & 1454.62 & 1476.37 & 1500.64 & 2965.79 & 1429.26 & \textbf{1389.64} & 1409.61 & 1408.93 & 1413.77 & 1417.12 & 1574.28            \\
%                               & IoU $\uparrow$    & 0.8552  & \textbf{0.8564}  & 0.8525  &             \\
% \midrule
% \multirow{2}{*}{Single-view}  & LFD $\downarrow$ & 2892.78 & \textbf{2885.85} & 2942.61 & 3166.60 & 2906.67 & 2894.96 & 2891.91 & 2911.02 & 2900.16 & 2923.45 & 2908.45 \\
%                               & IoU $\uparrow$   & \textbf{0.5961}  & 0.5934  & 0.5733  &                \\
% \midrule
% \multirow{2}{*}{Multi-view}   & LFD $\downarrow$ & 1585.10 & 1564.41 & 1556.83 & 2371.45 & & \textbf{1507.04} & 1538.63 & 1525.69 & 1529.07 & 1527.60 &               \\
%                               & IoU $\uparrow$   & \textbf{0.81098} & 0.8083  & 0.7960 &                \\
% \midrule
% \multirow{2}{*}{Voxels ()}    & LFD $\downarrow$ & 1970.10 & 1949.43 & 2035.14 & 2449.85 & 1935.44 & 1906.15 & 1931.36 & 1939.85 & 1932.56 & 1950.61 & \textbf{1872.56}                \\
%                               & IoU $\uparrow$   & 0.7454  & \textbf{0.7457}  & 0.7307  &                \\
% \midrule
% \multirow{2}{*}{4 depth}      & LFD $\downarrow$ & & & & 2430.07 & & \textbf{1414.29} & 1408.15 & 1421.16 & 1420.80 & 1428.63  \\
%                               & IoU $\uparrow$   & & & &               \\
% \midrule
% \multirow{2}{*}{6 depth}      & LFD $\downarrow$ & & & & 2588.48 & & \textbf{1348.32} & 1350.47 & 1353.88 & 1355.54& 1360.20 \\
%                               & IoU $\uparrow$   \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}[htbp]
\centering
 % Adjusts the size to be smaller
 {\smaller
 \caption{Performance metrics across different input modalities at various time steps.}

\begin{tabular}{c|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textit{Timestep}} & \multicolumn{2}{c|}{\textit{6 views depth}} & \multicolumn{2}{c|}{\textit{pointcloud}} & \multicolumn{2}{c|}{\textit{voxel 16}} & \multicolumn{2}{c|}{\textit{multiview}} & \multicolumn{2}{c}{\textit{singleview}} \\

 & IOU $\uparrow$ & LFD $\downarrow$ & IOU $\uparrow$ & LFD $\downarrow$ & IOU $\uparrow$ & LFD $\downarrow$ & IOU $\uparrow$ & LFD $\downarrow$ & IOU $\uparrow$ & LFD $\downarrow$ \\
\midrule
5   & 0.8587 & 1359.44 & 0.8600 & 1437.93 & \textbf{0.7570} & \textbf{1858.22} & \textbf{0.8191} & \underline{1484.63} & \textbf{0.5992} & 2968.87 \\
7   & 0.8597 & 1344.70 & 0.8629 & 1401.67 & 0.7512 & 1861.22 & 0.8166 & 1496.30 & 0.5985 & 2902.46 \\
8   & 0.8599 & 1334.32 & \textbf{0.8635} & 1392.32 & 0.7493 & 1883.12 & 0.8166 & 1505.45 & 0.5953 & 2917.60 \\
10  & \textbf{0.8601} & 1331.21 & 0.8624 & 1398.52 & 0.7482 & 1872.10 & 0.8139 & 1495.95 & 0.5933 & \textbf{2869.81} \\
12  & 0.8596 & \textbf{1330.09} & 0.8629 & 1392.21 & 0.7448 & 1916.72 & 0.8109 & \textbf{1483.51} & 0.5882 & 2894.04 \\
15  & 0.8590 & 1332.01 & 0.8617 & \textbf{1387.60} & 0.7414 & 1894.60 & 0.8121 & 1487.45 & 0.5828 & 2916.25 \\
18  & 0.8578 & 1337.51 & 0.8623 & 1398.98 & 0.7417 & 1902.33 & 0.8079 & 1496.62 & 0.5854 & 2922.46 \\
20  & 0.8574 & 1332.84 & 0.8588 & 1400.42 & 0.7397 & 1940.50 & 0.8058 & 1498.59 & 0.5833 & 2918.72 \\
25  & 0.8564 & 1345.35 & 0.8611 & 1399.75 & 0.7330 & 1944.23 & 0.8085 & 1504.62 & 0.5808 & 2933.45 \\
50  & 0.8537 & 1349.43 & 0.8551 & 1417.89 & 0.7301 & 1950.85 & 0.8003 & 1515.53 & 0.5731 & 2942.72 \\
100 & 0.8489 & 1368.77 & 0.8539 & 1412.05 & 0.7248 & 1987.58 & 0.7905 & 1535.27 & 0.5651 & 2955.67 \\
\bottomrule
\end{tabular}
}
\end{table}




